Disc fragmentation and oligarchic growth of protostellar systems in low-metallicity gas clouds

We study low-metallicity star formation with a set of high-resolution hydrodynamics simulations for various gas metallicities over a wide range $0$--$10^{-3} \ {\rm Z}_{\bigodot}$. Our simulations follow non-equilibrium chemistry and radiative cooling by adopting realistic elemental abundance and dust size distribution. We examine the condition for the fragmentation of collapsing clouds (cloud fragmentation; CF) and of accretion discs (disc fragmentation; DF). We find that CF is suppressed due to rapid gas heating accompanied with molecular hydrogen formation even with efficient dust cooling for metallicities $\gtrsim 10^{-5} \ {\rm Z}_{\bigodot}$. Instead, DF occurs in almost all runs regardless of metallicity. We also find that, in the accretion discs, the growth of the protostellar systems is overall oligarchic. The primary protostar grows through the accretion of gas, and secondary protostars form through the interaction of spiral arms or the break-up of a rapidly rotating protostar. Despite vigorous fragmentation, a large fraction of secondary protostars are destroyed through mergers or tidal disruption events. For a few hundred years after the first adiabatic core formation, only several protostars survive in the disc, and the total mass of protostars is $0.52$--$3.8 \ {\rm M}_{\bigodot}$.

==> table.tex <==
\begin{table*}
\begin{minipage}{15cm}
\caption{Properties of protostars for Halo A}
\label{tab:PSs_HA}
\begin{tabular}{cccccccccccccc}
\hline
 $Z$       & $i$ & $t_{\rm form}$ & form  &parent & $t_{\rm dest}$ & dest. & $j$  & $b$  &  $a_j$    & $m_j/m_i$& $r_{\rm tid}$ & $t_{\rm life}$ &     $M_*$   \\
 $[\Zsun]$ &     & [yr]           &       &       & [yr]           &       &      & [au] &  [au]     &          & [au]          & [yr]           & [$\Msun$]   \\
\hline \hline                                                                                                   
 $10^{-3}$ &   1 &            2.7 &    GC &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.471  \\
           &   2 &          368.7 &   INT &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.025  \\
           &   3 &          383.3 &   INT &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.026  \\
\hline                                                                                                                                   
 $10^{-4}$ &   1 &            1.5 &    GC &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.328  \\
           &   2 &          114.3 &    BU &    1  &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.097  \\
           &   3 &          128.7 &   INT &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.142  \\
\hline                                                                                                                                   
 $10^{-5}$ &   1 &            0.9 &    GC &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.584  \\
           &   2 &           35.9 &   INT &   --- &           39.1 &   MER &   1  & 3.72 &      4.22 &     53.07&         15.87 &            3.2 & (    0.005) \\
           &   3 &           59.7 &   INT &   --- &           92.3 &   MER &   4  & 0.13 &      1.05 &      3.39&          1.57 &           32.6 & (    0.037) \\
           &   4 &           60.9 &    BU &    1  &          137.1 &   TDE &   1  & 3.82 &      2.03 &      1.44&          2.30 &           76.2 & (    0.283) \\
           &   5 &           68.7 &   INT &   --- &           80.9 &   TDE &   4  & 1.16 &      0.74 &      3.73&          1.15 &           12.2 & (    0.020) \\
           &   6 &           71.7 &   INT &   --- &          145.7 &   TDE &   8  & 3.03 &      1.51 &      1.63&          1.78 &           74.0 & (    0.110) \\
           &   7 &           75.3 &   INT &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.140  \\
           &   8 &          141.5 &    BU &    1  &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.309  \\
\hline                                                                                                                                   
 $10^{-6}$ &   1 &            0.3 &    GC &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.795  \\
           &   2 &           53.9 &    BU &    1  &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.580  \\
           &   3 &           87.1 &   INT &   --- &           89.5 &   MER &   2  & 1.00 &      1.19 &      7.57&          2.33 &            2.4 & (    0.016) \\
           &   4 &           89.3 &   INT &   --- &           90.9 &   TDE &   2  & 1.59 &      1.48 &      8.29&          3.00 &            1.6 & (    0.018) \\
           &   5 &          114.9 &    BU &    1  &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.032  \\
\hline                                                                                                                                   
 0         &   1 &            0.3 &    GC &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      1.782  \\
           &   2 &            3.1 &    GC &   --- &            3.3 &   MER &   1  & 0.00 &      4.13 &     17.87&         10.79 &            0.2 & (    0.005) \\
           &   3 &            3.3 &    GC &   --- &            7.7 &   MER &   1  & 0.61 &      1.27 &      4.51&          2.10 &            4.4 & (    0.044) \\
           &   4 &            4.9 &    GC &   --- &            6.3 &   MER &   1  & 0.32 &      1.11 &      9.66&          2.37 &            1.4 & (    0.016) \\
           &   5 &            4.9 &    GC &   --- &           11.7 &   MER &   1  & 0.87 &      1.39 &      2.96&          1.99 &            6.8 & (    0.107) \\
           &   6 &            8.5 &    GC &   --- &           13.5 &   MER &   1  & 1.02 &      2.63 &     26.32&          7.83 &            5.0 & (    0.017) \\
           &   7 &           11.9 &    GC &   --- &           15.7 &   MER &   1  & 1.36 &      2.14 &     17.50&          5.55 &            3.8 & (    0.029) \\
           &   8 &           87.9 &    BU &    1  &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.712  \\
           &   9 &          112.7 &   INT &   --- &          123.5 &   DIS & ---  & 5.26 &      4.01 &     20.30&         10.93 &           10.8 & (    0.078) \\
           &  10 &          117.1 &   INT &   --- &          163.1 &   TDE &   1  & 5.64 &      4.16 &     15.11&         10.29 &           46.0 & (    0.110) \\
           &  11 &          123.7 &    GC &   --- &          123.9 &   TDE &   1  & 0.49 &      4.11 &     20.36&         11.23 &            0.2 & (    0.077) \\
           &  12 &          137.1 &   INT &   --- &          154.1 &   MER &   8  & 0.22 &      1.05 &      2.56&          1.44 &           17.0 & (    0.111) \\
           &  13 &          168.5 &    BU &    1  &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.103  \\
\hline
\end{tabular}
\medskip \\
Note --- 
(1) Metallicity $Z$.
(2) ID of a protostar $i$. 
(3) Formation time $t_{\rm form}$ of protostars.
(4) Formation paths of each protostar: 
gravitational contraction (GC),
break-up of a parent protostar (BU), and 
interaction of spiral arms \textcolor{red}{(INT)}.
(5) ID of the parent protostar which breaks up.
(6) Destruction time $t_{\rm dest}$ of protostars.
(7) Destruction mechanism: 
merger (MER),
tidal disruption event (TDE), and
dissolution to the ambient gas (DIS).
(8) ID of counterpart $j$ with which the protostar $i$ interacts.
(9-12) Impact parameter $b$, 
radius of major-axis $r_j$, mass radio $m_j/m_i$, and tidal radius $r_{\rm tid}$ 
of the impactor $j$.
(13) Life time $t_{\rm life}$ of the protostar.
(14) protostellar mass $M_*$ when it is destroyed with parentheses or
when the simulation is terminated at $t_{*,{\rm fin}}$ without parentheses.
\end{minipage}
\end{table*}


\begin{table*}
\begin{minipage}{15cm}
\caption{Properties of protostars for Halo B}
\label{tab:PSs_HB}
\begin{tabular}{cccccccccccccc}
\hline
 $Z$       & $i$ & $t_{\rm form}$ & form  &parent & $t_{\rm dest}$ & dest. & $j$  & $b$  &  $a_j$    & $m_j/m_i$& $r_{\rm tid}$ & $t_{\rm life}$ &     $M_*$   \\
 $[\Zsun]$ &     & [yr]           &       &       & [yr]           &       &      & [au] &  [au]     &          & [au]          & [yr]           & [$\Msun$]   \\
\hline \hline                                                                                                   
 $10^{-3}$ &   1 &            0.7 &    GC &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      1.407  \\
           &   2 &          178.9 &    BU &    1  &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.015  \\
\hline                                                                                                                                 
 $10^{-4}$ &   1 &            1.3 &    GC &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      1.693  \\
           &   2 &           52.3 &   INT &   --- &           67.9 &   MER &   1  & 5.96 &      6.46 &     28.11&         19.63 &           15.6 & (    0.044) \\
           &   3 &           69.9 &    GC &   --- &           70.1 &   DIS & ---  & 0.00 &      5.20 &    280.10&         34.00 &            0.2 & (    0.005) \\
           &   4 &           73.5 &    BU &    1  &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.018  \\
           &   5 &           78.5 &    BU &    1  &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.156  \\
           &   6 &           87.5 &   INT &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.012  \\
           &   7 &           90.1 &   INT &   --- &           95.1 &   TDE &   1  & 5.83 &      4.21 &    328.25&         29.06 &            5.0 & (    0.005) \\
           &   8 &           92.5 &   INT &   --- &           93.5 &   TDE &   1  & 5.85 &      3.74 &    287.93&         24.68 &            1.0 & (    0.005) \\
           &   9 &           94.5 &    BU &    1  &           94.7 &   MER &   1  & 0.84 &      4.11 &    420.29&         30.81 &            0.2 & (    0.004) \\
\hline                                                                                                                                 
 $10^{-5}$ &   1 &            0.5 &    GC &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      1.076  \\
           &   2 &           42.5 &    BU &    1  &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.393  \\
           &   3 &           42.7 &   INT &   --- &           46.9 &   TDE &   1  & 3.11 &      2.52 &     76.74&         10.71 &            4.2 & (    0.009) \\
           &   4 &           52.3 &   INT &   --- &           87.1 &   TDE &   1  & 3.15 &      3.07 &     21.49&          8.54 &           34.8 & (    0.045) \\
           &   5 &           54.5 &   INT &   --- &           67.9 &   TDE &   2  & 1.38 &      1.25 &     16.93&          3.20 &           13.4 & (    0.010) \\
           &   6 &           58.7 &   INT &   --- &           66.7 &   TDE &   2  & 1.35 &      1.13 &     10.96&          2.52 &            8.0 & (    0.015) \\
           &   7 &           69.3 &   INT &   --- &           83.7 &   TDE &   2  & 1.57 &      1.25 &     20.51&          3.41 &           14.4 & (    0.013) \\
           &   8 &           82.3 &   INT &   --- &           94.5 &   MER &   1  & 1.64 &      3.78 &     41.05&         13.03 &           12.2 & (    0.025) \\
           &   9 &           83.9 &   INT &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.011  \\
           &  10 &           89.1 &    BU &    1  &           89.7 &   DIS & ---  & 4.44 &      3.14 &    317.30&         21.45 &            0.6 & (    0.003) \\
           &  11 &           93.3 &    GC &   --- &           94.5 &   DIS & ---  &11.55 &      3.78 &    330.92&         26.12 &            1.2 & (    0.003) \\
           &  12 &           94.7 &    GC &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.005  \\
           &  13 &           99.1 &    BU &    1  &           99.5 &   DIS & ---  & 4.46 &      3.59 &    196.66&         20.86 &            0.4 & (    0.005) \\
\hline                                                                                                                                 
 $10^{-6}$ &   1 &            0.5 &    GC &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      5.615  \\
           &   2 &            8.3 &    GC &   --- &           11.7 &   MER &   1  & 1.17 &      1.99 &      9.60&          4.23 &            3.4 & (    0.078) \\
           &   3 &            9.5 &    GC &   --- &           13.1 &   MER &   1  & 1.80 &      2.55 &     15.96&          6.43 &            3.6 & (    0.057) \\
           &   4 &           11.5 &    GC &   --- &           14.5 &   TDE &   1  & 2.62 &      2.24 &     25.98&          6.65 &            3.0 & (    0.039) \\
\hline                                                                                                                                 
 0         &   1 &            0.3 &    GC &   --- &           10.3 &   TDE &   2  & 3.70 &      2.06 &      1.15&          2.15 &           10.0 & (    0.365) \\
           &   2 &            4.3 &   INT &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      2.113  \\
           &   3 &           32.1 &   INT &   --- &           35.5 &   TDE &   2  & 3.92 &      2.61 &     16.01&          6.57 &            3.4 & (    0.056) \\
           &   4 &           32.5 &   INT &   --- &           36.3 &   MER &   7  & 0.76 &      0.77 &      0.32&          1.25 &            3.8 & (    0.036) \\
           &   5 &           32.7 &   INT &   --- &           39.1 &   TDE &   2  & 3.42 &      2.97 &      5.89&          5.36 &            6.4 & (    0.167) \\
           &   6 &           33.1 &    BU &    5  &           33.3 &   MER &   5  & 1.06 &      2.18 &      3.29&          3.25 &            0.2 & (    0.005) \\
           &   7 &           35.9 &   INT &   --- &           36.3 &   MER &   4  & 0.76 &      0.86 &      3.08&          1.25 &            0.4 & (    0.012) \\
           &   8 &           37.3 &    BU &    5  &           40.9 &   MER &  13  & 0.66 &      0.67 &      1.49&          0.77 &            3.6 & (    0.024) \\
           &   9 &           37.5 &   INT &   --- &           49.3 &   TDE &  13  & 3.87 &      3.73 &      3.88&          5.86 &           11.8 & (    0.133) \\
           &  10 &           37.5 &   INT &   --- &           47.7 &   TDE &  13  & 4.31 &      2.16 &      1.16&          2.27 &           10.2 & (    0.203) \\
           &  11 &           38.1 &    BU &    2  &           47.1 &   MER &  10  & 2.05 &      2.51 &      3.24&          3.71 &            9.0 & (    0.045) \\
           &  12 &           38.3 &   INT &   --- &           45.5 &   TDE &   9  & 1.88 &      0.90 &      2.77&          1.26 &            7.2 & (    0.031) \\
           &  13 &           38.9 &   INT &   --- &           66.5 &   TDE &   2  & 5.71 &      2.80 &      1.71&          3.35 &           27.6 & (    0.855) \\
           &  14 &           40.5 &   INT &   --- &           45.3 &   TDE &  13  & 1.24 &      1.05 &      0.98&          1.03 &            4.8 & (    0.097) \\
           &  15 &           40.5 &   INT &   --- &           49.3 &   MER &   2  & 3.22 &      4.10 &    305.09&         27.59 &            8.8 & (    0.004) \\
           &  16 &           41.1 &    BU &    2  &           41.7 &   TDE &  15  & 5.21 &      1.26 &      7.53&          2.47 &            0.6 & (    0.003) \\
           &  17 &           42.1 &   INT &   --- &           43.3 &   TDE &  15  & 5.49 &      0.90 &     12.91&          2.12 &            1.2 & (    0.004) \\
           &  18 &           42.7 &    BU &   11  &           43.7 &   TDE &  10  & 1.92 &      1.50 &      3.48&          2.28 &            1.0 & (    0.023) \\
           &  19 &           43.9 &   INT &   --- &           49.9 &   MER &   2  & 3.48 &      4.10 &     48.15&         14.91 &            6.0 & (    0.027) \\
           &  20 &           47.5 &   INT &   --- &           59.9 &   TDE &   2  & 4.84 &      4.33 &     12.93&         10.16 &           12.4 & (    0.109) \\
           &  21 &           51.5 &   INT &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.352  \\
           &  22 &           65.9 &   INT &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.126  \\
           &  23 &           69.9 &   INT &   --- &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.815  \\
           &  24 &           70.7 &    BU &    2  &            --- &   --- & ---  &  --- &       --- &       ---&           --- &            --- &      0.365  \\
           &  25 &           71.5 &   INT &   --- &           73.9 &   TDE &  22  & 1.50 &      0.94 &      2.54&          1.28 &            2.4 & (    0.022) \\
           &  26 &           75.3 &   INT &   --- &           82.5 &   MER &  23  & 1.02 &      1.56 &      3.44&          2.36 &            7.2 & (    0.121) \\
\hline
\end{tabular}
\medskip \\
\end{minipage}
\end{table*}

